Constraints on the Initial-Final Mass Relation from Wide Double White Dwarfs

We present observational constraints on the initial-final mass relation (IFMR) using wide double white dwarfs (DWDs). We identify 65 new candidate wide DWDs within the Sloan Digital Sky Survey, bringing the number of candidate wide DWDs to 142. We then engage in a spectroscopic follow-up campaign and collect existing spectra for these objects; using these spectra, we derive masses and cooling ages for 54 hydrogen (DA) WDs in DWDs. We also identify one new DA/DB pair, four candidate DA/DC pairs, four candidate DA/DAH pairs, and one new candidate triple degenerate system. Because wide DWDs are co-eval and evolve independently, the difference in the pre-WD lifetimes should equal the difference in the WD cooling ages. We use this to develop a Bayesian hierarchical framework and construct a likelihood function to determine the probability that any particular IFMR fits a sample of wide DWDs. We then define a parametric model for the IFMR and find the best parameters indicated by our sample of DWDs. We place robust constraints on the IFMR for initial masses of 2--4 \Msun. The WD masses produced by our model for stars within this mass range differ from those predicted by semi-empirical fits to open cluster WDs. Within this mass range, where there are few constraining open cluster WDs and disagreements in the cluster ages, wide DWDs may provide more reliable constraints on the IFMR. Expanding this method to the many wide DWDs expected to be discovered by Gaia may transform our understanding of the IFMR.

==> table2_full.tex <==
\begin{deluxetable*}{lllllllcl}
\tablecaption{Wide Double White Dwarf -- Observed Quantities \label{tab:DWD_obs}}
\tablehead{
\colhead{Name} & 
\colhead{$\alpha$} & 
\colhead{$\delta$} & 
\colhead{$g$} & 
\colhead{$\mu_{\alpha}$} & 
\colhead{$\mu_{\delta}$} & 
\colhead{$\theta$} &
\colhead{Targeted for} &
\colhead{Source} \\ 
\colhead{} & 
\colhead{} & 
\colhead{} & 
\colhead{(mag)} & 
\colhead{(mas yr$^{-1}$)} & 
\colhead{(mas yr$^{-1}$)} & 
\colhead{(\asec)} &
\colhead{Spectroscopy} &
\colhead{}
}

\startdata 
\multirow{2}{*}{J0000-0308}  &  00:00:11.63  &  -03:08:31.88  &  20.11 $\pm$ 0.02  &  42.43 $\pm$ 3.25  &  -21.97 $\pm$ 3.25  &  \multirow{2}{*}{6.1} & \multirow{2}{*}{N} & \multirow{2}{*}{1} \\
 &  00:00:12.04  &  -03:08:31.34  &  20.01 $\pm$ 0.02  &  48.15 $\pm$ 3.25  &  -21.02 $\pm$ 3.25  & & &\\
 
\multirow{2}{*}{J0000-1051}  &  00:00:22.53  &  -10:51:42.12  &  18.90 $\pm$ 0.01  &  45.26 $\pm$ 4.65  &  -23.81 $\pm$ 4.65  &  \multirow{2}{*}{16.1} & \multirow{2}{*}{N} & \multirow{2}{*}{2} \\
 &  00:00:22.83  &  -10:51:26.64  &  20.21 $\pm$ 0.02  &  42.37 $\pm$ 4.08  &  -23.57 $\pm$ 4.08  & & &\\
 
\multirow{2}{*}{CDDS1 } & 00:01:42.84 & +25:15:06.1  &  17.79 $\pm$ 0.02  &  &  & \multirow{2}{*}{2.16} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 00:01:42.79 & +25:15:04.0  &  18.70 $\pm$ 0.16  &  & & & & \\ 
 
\multirow{2}{*}{J0002+0733}  &  00:02:15.33  &  +07:33:59.14  &  17.85 $\pm$ 0.01  &  -103.4 $\pm$ 2.77  &  -64.37 $\pm$ 2.77  &  \multirow{2}{*}{15.1} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  00:02:16.13  &  +07:33:49.93  &  18.07 $\pm$ 0.01  &  -103.62 $\pm$ 2.85  &  -63.59 $\pm$ 2.85  & & &\\
 
\multirow{2}{*}{J0029+0015}  &  00:29:25.29  &  +00:15:59.79  &  19.59 $\pm$ 0.01  &  -27.87 $\pm$ 3.62  &  -23.24 $\pm$ 3.62  &  \multirow{2}{*}{8.7} & \multirow{2}{*}{N} & \multirow{2}{*}{2,3}\\
 &  00:29:25.62  &  +00:15:52.72  &  18.46 $\pm$ 0.01  &  -28.33 $\pm$ 3.13  &  -22.58 $\pm$ 3.13  && & \\
 
\multirow{2}{*}{J0030+1810}  &  00:30:51.75  &  +18:10:53.75  &  18.72 $\pm$ 0.01  &    &    &  \multirow{2}{*}{7.8} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  00:30:51.80  &  +18:10:46.05  &  18.73 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{CDDS3 } & 00:52:12.26 & +13:53:02.0  &  17.71 $\pm$ 0.03  &  &  & \multirow{2}{*}{6.78} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 00:52:12.73 & +13:53:01.1  &  18.89 $\pm$ 0.03  &  & & & & \\ 
 
\multirow{2}{*}{LP 406-62/63}  &  01:04:56.33  &  +21:19:54.9  &  18.30 $\pm$ 0.02  &  -210.33 $\pm$ 2.51  &  -431.2 $\pm$ 2.51  &  \multirow{2}{*}{28} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  01:04:57.81  &  +21:20:13.49  &  18.59 $\pm$ 0.02  &  -209.48 $\pm$ 2.62  &  -436.89 $\pm$ 2.62  & & &\\
 
\multirow{2}{*}{J0105-0741}  &  01:05:53.78  &  -07:41:22.19  &  20.51 $\pm$ 0.03  &  -47.73 $\pm$ 4.65  &  -66.24 $\pm$ 4.65  &  \multirow{2}{*}{10} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  01:05:54.14  &  -07:41:30.84  &  18.57 $\pm$ 0.01  &  -48.41 $\pm$ 2.57  &  -61.63 $\pm$ 2.57  & & &\\
 
\multirow{2}{*}{J0107+0511}  &  01:07:17.20  &  +05:11:46.78  &  18.67 $\pm$ 0.01  &  -59.61 $\pm$ 2.86  &  -79.32 $\pm$ 2.86  &  \multirow{2}{*}{41.6} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  01:07:19.89  &  +05:11:58.09  &  20.54 $\pm$ 0.02  &  -49.86 $\pm$ 3.48  &  -73.05 $\pm$ 3.48  & & &\\
 
\multirow{2}{*}{LP707-8/9}  &  01:09:03.42  &  -10:42:14.17  &  16.77 $\pm$ 0.03  &  169.41 $\pm$ 2.65  &  -28.7 $\pm$ 2.65  &  \multirow{2}{*}{12} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  01:09:04.23  &  -10:42:15.45  &  19.45 $\pm$ 0.04  &  170.79 $\pm$ 3.5  &  -25.88 $\pm$ 3.5  & & &\\
 
\multirow{2}{*}{J0117+2440}  &  01:17:14.13  &  +24:40:20.31  &  19.84 $\pm$ 0.01  &    &    &  \multirow{2}{*}{5} & \multirow{2}{*}{N} & \multirow{2}{*}{1,3}\\
 &  01:17:14.49  &  +24:40:21.46  &  19.62 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{LP647-33/34}  &  01:17:28.67  &  -04:39:40.84  &  18.52 $\pm$ 0.04  &    &    &  \multirow{2}{*}{2} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  01:17:28.48  &  -04:39:42.12  &  18.68 $\pm$ 0.03  &    &    & & &\\
 
\multirow{2}{*}{CDDS5 } & 01:27:26.89 & +39:15:03.3  &  18.70 $\pm$ 0.02  &  &  & \multirow{2}{*}{16.55} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 01:27:25.51 & +39:14:59.2  &  19.99 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{J0133+3011}  &  01:33:10.11  &  +30:11:53.7  &  19.19 $\pm$ 0.01  &    &    &  \multirow{2}{*}{7.7} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  01:33:10.69  &  +30:11:52.61  &  19.68 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{J0136+3048}  &  01:36:32.28  &  +30:48:14.97  &  20.14 $\pm$ 0.03  &    &    &  \multirow{2}{*}{3}  & \multirow{2}{*}{N} &\multirow{2}{*}{1}\\
 &  01:36:32.46  &  +30:48:16.73  &  20.07 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{J0138+5559}  &  01:38:19.05  &  +55:59:40.55  &  19.70 $\pm$ 0.01  &  15.99 $\pm$ 4.79  &  -65.7 $\pm$ 4.79  &  \multirow{2}{*}{10.9} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  01:38:19.96  &  +55:59:32.99  &  19.68 $\pm$ 0.01  &  21.28 $\pm$ 3.38  &  -60.16 $\pm$ 3.38  & & &\\
 
\multirow{2}{*}{J0139+1447}  &  01:39:10.70  &  +14:47:26.51  &  19.55 $\pm$ 0.01  &  -19.82 $\pm$ 3.62  &  -47.44 $\pm$ 3.62  &  \multirow{2}{*}{68.4} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  01:39:11.01  &  +14:48:34.91  &  19.64 $\pm$ 0.01  &  -22.61 $\pm$ 5  &  -40.87 $\pm$ 5  & & &\\
 
\multirow{2}{*}{J0211+1714}  &  02:11:31.51  &  +17:14:30.44  &  17.20 $\pm$ 0.01  &    &    &  \multirow{2}{*}{2.1} & \multirow{2}{*}{N} & \multirow{2}{*}{1,3}\\
 &  02:11:31.52  &  +17:14:28.31  &  16.76 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{LP 197-5/6}  &  02:25:51.96  &  +42:28:04.3  &      &    &    &  \multirow{2}{*}{7} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  02:25:52.59  &  +42:28:05.56  &      &    &    & & &\\
 
\multirow{2}{*}{CDDS7 } & 02:27:33.09 & +00:52:00.3  &  19.62 $\pm$ 0.02  &  &  & \multirow{2}{*}{6.72} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 02:27:33.15 & +00:51:53.6  &  19.86 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{J0304+4541}  &  03:04:29.38  &  +45:41:48.15  &  20.09 $\pm$ 0.02  &    &    &  \multirow{2}{*}{6.5} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  03:04:30.00  &  +45:41:47.83  &  19.41 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J0316+0319}  &  03:16:29.61  &  +03:18:58.03  &  20.28 $\pm$ 0.02  &  -15.31 $\pm$ 4.66  &  -42.48 $\pm$ 4.66  &  \multirow{2}{*}{20.5} & \multirow{2}{*}{N} &  \multirow{2}{*}{1}\\
 &  03:16:30.93  &  +03:19:04.36  &  18.14 $\pm$ 0.01  &  -12.62 $\pm$ 2.65  &  -35.44 $\pm$ 2.65  & & &\\
 
\multirow{2}{*}{RE J0317-853}  &  03:17:16.18  &  -85:32:25.45  &      &    &    &  \multirow{2}{*}{7} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  03:17:19.31  &  -85:32:31.15  &      &    &    & & &\\
 
\multirow{2}{*}{LP 472-70/69}  &  03:25:38.33  &  +15:09:00.89  &      &    &    &  \multirow{2}{*}{3} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  03:25:36  &  +15:08.5  &      &    &    & & &\\
 
\multirow{2}{*}{J0332-0049}  &  03:32:36.59  &  -00:49:18.42  &      &  -24.79 $\pm$ 5.39  &  -23.63 $\pm$ 5.39  &  \multirow{2}{*}{19} & \multirow{2}{*}{N} & \multirow{2}{*}{2,3}\\
 &  03:32:36.86  &  -00:49:36.93  &      &  -30.91 $\pm$ 4.48  &  -23.31 $\pm$ 4.48  & & &\\
 
\multirow{2}{*}{J0344+1510}  &  03:44:10.91  &  +15:10:22.08  &  16.52 $\pm$ 0.01  &  21.42 $\pm$ 2.53  &  -36.7 $\pm$ 2.53  &  \multirow{2}{*}{37.5} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  03:44:11.49  &  +15:09:45.71  &  16.89 $\pm$ 0.01  &  23.79 $\pm$ 2.56  &  -40.62 $\pm$ 2.56  & & &\\
 
\multirow{2}{*}{HS 0507+0434}  &  05:10:13.52  &  +04:38:55.2  &      &    &    &  \multirow{2}{*}{18} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  05:10:14.0  &  +04:38:41  &      &    &    & & &\\
 
\multirow{2}{*}{LMC 102.7.22886(769)}  &  05:18:51.10  &  -68:11:17.7  &      &    &    &  \multirow{2}{*}{96.3} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  05:18:54.98  &  -68:09:48.3  &      &    &    & & &\\
 
\multirow{2}{*}{CDDS9 } & 05:45:19.81 & +30:27:54.0  &  19.82 $\pm$ 0.02  &  &  & \multirow{2}{*}{11.72} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 05:45:18.98 & +30:27:49.3  &  19.64 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{CDDS10 } & 07:21:47.38 & +32:28:24.1  &  18.07 $\pm$ 0.01  &  &  & \multirow{2}{*}{2.77} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 07:21:47.20 & +32:28:22.4  &  18.32 $\pm$ 0.06  &  & & & & \\ 
 
\multirow{2}{*}{J0729+6519}  &  07:29:19.15  &  +65:19:10.88  &  20.88 $\pm$ 0.03  &  0   &  0   &  \multirow{2}{*}{9.1} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  07:29:20.61  &  +65:19:10.34  &  20.79 $\pm$ 0.02  &  0  &  0  & & &\\
 
\multirow{2}{*}{WD0727+482A/B}  &  07:30:42.80  &  +48:12:00.0  &      &    &    &  & \multirow{2}{*}{N} &  \multirow{2}{*}{4}\\
 &  07:30:47.36  &  +48:10:27.6  &      &    &    & & &\\
 
\multirow{2}{*}{J0748+3025}  &  07:48:52.96  &  +30:25:43.42  &  17.73 $\pm$ 0.01  &    &    &  \multirow{2}{*}{1.5} & \multirow{2}{*}{N} & \multirow{2}{*}{1,3}\\
 &  07:48:53.08  &  +30:25:43.57  &  17.41 $\pm$ 0.01  &    &   & & &\\
 
\multirow{2}{*}{LP543-33/32}  &  07:50:15.42  &  +07:11:26.64  &  17.20 $\pm$ 0.02  &  209.72 $\pm$ 2.53  &  -1787.91 $\pm$ 2.53  &  \multirow{2}{*}{16} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  07:50:14.67  &  +07:11:38.5  &  17.64 $\pm$ 0.02  &  208.92 $\pm$ 2.59  &  -1783.09 $\pm$ 2.59  & & &\\
 
\multirow{2}{*}{J0754+1239}  &  07:54:10.53  &  +12:39:47.41  &  18.73 $\pm$ 0.01  &    &    &  \multirow{2}{*}{2} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  07:54:10.58  &  +12:39:45.53  &  18.83 $\pm$ 0.01  &   0  &  0  & & &\\
 
\multirow{2}{*}{J0754+4950}  &  07:54:20.88  &  +49:50:05.28  &  20.61 $\pm$ 0.03  &  -16.59 $\pm$ 5.41  &  -60.3 $\pm$ 5.41  &  \multirow{2}{*}{11} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  07:54:21.11  &  +49:50:16.43  &  19.46 $\pm$ 0.01  &  -23.46 $\pm$ 3.54  &  -64.35 $\pm$ 3.54  & & &\\
 
\multirow{2}{*}{CDDS13 } & 08:02:12.54 & +24:20:43.6  &  19.54 $\pm$ 0.02  &  &  & \multirow{2}{*}{25.85} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 08:02:13.44 & +24:20:20.9  &  19.84 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{CDDS14 } & 08:06:44.09 & +44:45:03.2  &  18.14 $\pm$ 0.02  &  &  & \multirow{2}{*}{5.09} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 08:06:43.64 & +44:45:01.4  &  18.74 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{J0827-0216}  &  08:27:30.57  &  -02:16:20.16  &  17.83 $\pm$ 0.01  &    &    &  \multirow{2}{*}{2.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  08:27:30.72  &  -02:16:18.54  &  17.99 $\pm$ 0.01  &    &   & & &\\
 
\multirow{2}{*}{LP 035-288/287}  &  08:46:01.07  &  +69:44:38.85  &      &    &    &  \multirow{2}{*}{3}  & \multirow{2}{*}{N} &\multirow{2}{*}{4}\\
 &  08:46:01.21  &  +69:44:37.5  &      &    &    & & &\\
 
\multirow{2}{*}{J0849+4712}  &  08:49:52.46  &  +47:12:47.73  &  17.70 $\pm$ 0.01  &    &   &  \multirow{2}{*}{4.4} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  08:49:52.87  &  +47:12:49.46  &  16.71 $\pm$ 0.01  &  -53.95 $\pm$ 2.64  &  -67.86 $\pm$ 2.64  & & &\\
 
\multirow{2}{*}{J0859+3306}  &  08:59:15.02  &  +33:06:44.67  &  18.00 $\pm$ 0.01  &    &    &  \multirow{2}{*}{9.3} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  08:59:15.50  &  +33:06:37.62  &  18.69 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{CDDS17 } & 08:59:17.36 & +42:50:31.6  &  18.94 $\pm$ 0.05  &  &  & \multirow{2}{*}{4.39} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 08:59:17.23 & +42:50:27.4  &  18.38 $\pm$ 0.04  &  & & & & \\ 
 
\multirow{2}{*}{PG 0901+140}  &  09:04:02.78  &  +13:49:14.84  &  16.10 $\pm$ 0.00  &   &    &  \multirow{2}{*}{3.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{4}\\
 &  09:04:02.80  &  +13:49:11.13  &  16.73 $\pm$ 0.00  &   &    & & &\\
 
\multirow{2}{*}{PG 0922+162}  &  09:25:13.17  &  +16:01:45.4  &  17.12 $\pm$ 0.01  &   &   &  \multirow{2}{*}{4.5} & \multirow{2}{*}{N} & \multirow{2}{*}{1,3}\\
 &  09:25:13.48  &  +16:01:44.14  &  16.12 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J0926+1321}  &  09:26:46.88  &  +13:21:34.5  &  18.37 $\pm$ 0.15  &  -49.11 $\pm$ 3.9  &  -142.69 $\pm$ 3.9  &  \multirow{2}{*}{4.6} & \multirow{2}{*}{N} & \multirow{2}{*}{4,3}\\
 &  09:26:47.00  &  +13:21:38.4  &  18.45 $\pm$ 0.04  &  11.41 $\pm$ 2.69  &  -4.36 $\pm$ 2.69  & & &\\
 
\multirow{2}{*}{LP 462-56A/B}  &  09:37:00.0  &  -37:21:33  &      &    &    &  \multirow{2}{*}{4} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  09:37:00.0  &  -37:21:33  &      &    &    & & &\\
 
\multirow{2}{*}{LP 370-50/51}  &  09:45:07.92  &  +23:27:23.03  &  17.50 $\pm$ 0.01  &  -191.34 $\pm$ 2.42  &  -101.41 $\pm$ 2.42  &  \multirow{2}{*}{13.2} & \multirow{2}{*}{Y} & \multirow{2}{*}{4}\\
 &  09:45:08.63  &  +23:27:31.32  &  17.70 $\pm$ 0.01  &  -189.29 $\pm$ 2.44  &  -100.68 $\pm$ 2.44  & & &\\
 
\multirow{2}{*}{CDDS20 } & 09:54:58.73 & +39:01:04.6  &  19.86 $\pm$ 0.02  &  &  & \multirow{2}{*}{18.87} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 09:54:59.97 & +39:00:52.4  &  17.69 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{J1002+3606}  &  10:02:44.87  &  +36:06:29.51  &  18.89 $\pm$ 0.01  &  -32.72 $\pm$ 3.29  &  -27.77 $\pm$ 3.29  &  \multirow{2}{*}{26.5} & \multirow{2}{*}{Y} & \multirow{2}{*}{2,3}\\
 &  10:02:45.83  &  +36:06:53.28  &  19.01 $\pm$ 0.01  &  -29.64 $\pm$ 3.44  &  -27.35 $\pm$ 3.44  & & &\\
 
\multirow{2}{*}{LP 549-33/32}  &  10:15:02.60  &  +08:06:35.7  &  16.19 $\pm$ 0.02  &  -288 $\pm$ 2.66  &  164.96 $\pm$ 2.66  &  \multirow{2}{*}{26} & \multirow{2}{*}{Y} &\multirow{2}{*}{4} \\
 &  10:15:01.73  &  +08:06:11.5  &  18.35 $\pm$ 0.02  &  -291.59 $\pm$ 3.03  &  155.47 $\pm$ 3.03  & & &\\
 
\multirow{2}{*}{PG 1017+125}  &  10:19:55.9  &  +12:16:31.48  &  15.51 $\pm$ 0.03  &  -24.14 $\pm$ 2.42  &  -18.03 $\pm$ 2.42  &  \multirow{2}{*}{48.8} & \multirow{2}{*}{Y} & \multirow{2}{*}{4}\\
 &  10:19:54.6  &  +12:17:17.98  &  16.75 $\pm$ 0.03  &  -27.02 $\pm$ 2.48  &  -23.99 $\pm$ 2.48  & & &\\
 
\multirow{2}{*}{J1048+0148}  &  10:48:18.59  &  +01:48:41.77  &  19.76 $\pm$ 0.02  &   &    &  \multirow{2}{*}{2.7} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  10:48:18.64  &  +01:48:44.34  &  19.69 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{CDDS22 } & 10:53:06.13 & +02:50:52.5  &  19.14 $\pm$ 0.02  &  &  & \multirow{2}{*}{26.60} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 10:53:06.82 & +02:50:27.9  &  18.98 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{LP 128-254/255}  &  10:54:49.1  &  +53:07:15.51  &  17.51 $\pm$ 0.02  &  -112.5 $\pm$ 2.95  &  -34.56 $\pm$ 2.95  &  \multirow{2}{*}{44} & \multirow{2}{*}{Y} & \multirow{2}{*}{4}\\
 &  10:54:49.88  &  +53:07:59.43  &  17.90 $\pm$ 0.02  &  -113.57 $\pm$ 3.1  &  -37.02 $\pm$ 3.1  & & &\\
 
\multirow{2}{*}{J1110+4517}  &  11:10:16.79  &  +45:17:36.23  &  17.67 $\pm$ 0.01  &  26.63 $\pm$ 2.87  &  -45.18 $\pm$ 2.87  &  \multirow{2}{*}{51.9} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  11:10:20.88  &  +45:18:01.79  &  16.80 $\pm$ 0.01  &  26.89 $\pm$ 3.61  &  -46.32 $\pm$ 3.61  & & &\\
 
\multirow{2}{*}{J1113+3238}  &  11:13:19.43  &  +32:38:17.88  &  19.03 $\pm$ 0.01  &  -162.09 $\pm$ 3.15  &  58.49 $\pm$ 3.15  &  \multirow{2}{*}{56.7} & \multirow{2}{*}{N} & \multirow{2}{*}{2}\\
 &  11:13:22.56  &  +32:38:58.92  &  19.11 $\pm$ 0.01  &  -158.09 $\pm$ 3.17  &  58.36 $\pm$ 3.17  & & &\\
 
\multirow{2}{*}{J1127+2725}  &  11:27:30.96  &  +27:25:42.95  &  20.81 $\pm$ 0.03  &    &    &  \multirow{2}{*}{8.6} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  11:27:31.68  &  +27:25:40.8  &  17.86 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{ESO 439-162/163}  &  11:29:52.04  &  -31:22:47.23  &      &    &    &  \multirow{2}{*}{23} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  11:29:53.79  &  -31:22:42.61  &      &    &    & & &\\
 
\multirow{2}{*}{J1130+2103}  &  11:30:32.97  &  +21:03:59.21  &  20.56 $\pm$ 0.03  &    &    &  \multirow{2}{*}{2.8} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  11:30:33.14  &  +21:03:57.99  &  20.29 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{CDDS23 } & 11:39:28.52 & -00:14:20.9  &  19.42 $\pm$ 0.02  &  &  & \multirow{2}{*}{2.95} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 11:39:28.47 & -00:14:18.0  &  19.80 $\pm$ 0.06  &  & & & & \\ 
 
\multirow{2}{*}{CDDS24 } & 11:50:30.12 & +25:32:10.1  &  19.95 $\pm$ 0.02  &  &  & \multirow{2}{*}{6.38} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 11:50:30.48 & +25:32:06.0  &  18.86 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{CDDS25 } & 11:53:05.54 & +00:56:46.1  &  18.89 $\pm$ 0.02  &  &  & \multirow{2}{*}{1.22} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 11:53:05.47 & +00:56:45.8  &  18.91 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{CDDS26 } & 11:59:37.81 & +13:44:13.9  &  18.07 $\pm$ 0.02  &  &  & \multirow{2}{*}{5.18} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 11:59:37.82 & +13:44:08.7  &  18.28 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{J1203+4948}  &  12:03:11.03  &  +49:48:50.76  &  17.33 $\pm$ 0.01  &  -97.34 $\pm$ 2.86  &  -40.44 $\pm$ 2.86  &  \multirow{2}{*}{19.3} & \multirow{2}{*}{Y} & \multirow{2}{*}{2}\\
 &  12:03:11.52  &  +49:48:32.39  &  19.01 $\pm$ 0.01  &  -96.7 $\pm$ 3.46  &  -37.92 $\pm$ 3.46  & & &\\
 
\multirow{2}{*}{CDDS27 } & 12:27:39.16 & +66:12:24.4  &  17.86 $\pm$ 0.02  &  &  & \multirow{2}{*}{11.43} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 12:27:41.05 & +66:12:24.3  &  17.99 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{J1230+4734}  &  12:30:21.81  &  +47:34:10.84  &  20.13 $\pm$ 0.02  &    &    &  \multirow{2}{*}{4.2} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  12:30:21.84  &  +47:34:06.63  &  19.90 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{J1231+5736}  &  12:31:55.72  &  +57:36:11.37  &  17.83 $\pm$ 0.01  &   &    &  \multirow{2}{*}{3.2} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  12:31:56.06  &  +57:36:09.75  &  18.53 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J1254-0218}  &  12:54:58.07  &  -02:18:37.8  &  16.46 $\pm$ 0.01  &  -12.57 $\pm$ 2.92  &  -55.89 $\pm$ 2.92  &  \multirow{2}{*}{30.8} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  12:54:58.55  &  -02:18:07.74  &  19.84 $\pm$ 0.02  &  -6.96 $\pm$ 4.04  &  -57.33 $\pm$ 4.04  & & &\\
 
\multirow{2}{*}{J1257+1925}  &  12:57:20.87  &  +19:25:03.71  &  19.86 $\pm$ 0.02  &  -39.68 $\pm$ 5.39  &  -31.27 $\pm$ 5.39  &  \multirow{2}{*}{12.2} & \multirow{2}{*}{N} & \multirow{2}{*}{2}\\
 &  12:57:21.12  &  +19:24:51.84  &  17.02 $\pm$ 0.01  &  -33.93 $\pm$ 2.74  &  -33.29 $\pm$ 2.74  & & &\\
 
\multirow{2}{*}{GD 322}  &  13:00:35.20  &  +59:04:15.6  &  15.24 $\pm$ 0.01  &  39.86 $\pm$ 2.62  &  73.37 $\pm$ 2.62  &  \multirow{2}{*}{16.1} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  13:00:33.46  &  +59:04:06.9  &  18.27 $\pm$ 0.01  &  39.1 $\pm$ 3.03  &  72.26 $\pm$ 3.03  & & &\\
 
\multirow{2}{*}{J1304+0917}  &  13:04:07.67  &  +09:17:22.84  &  20.43 $\pm$ 0.03  &  -48.29 $\pm$ 3.63  &  8.04 $\pm$ 3.63  &  \multirow{2}{*}{23.3} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  13:04:08.64  &  +09:17:41.1  &  19.99 $\pm$ 0.02  &  -49.11 $\pm$ 3.48  &  6.89 $\pm$ 3.48  & & &\\
 
\multirow{2}{*}{LP 322-500A/B}  &  13:04:29.42  &  +30:59:00.39  &  18.58 $\pm$ 0.03  &  -0.36 $\pm$ 3.11  &  -16.95 $\pm$ 3.11  &  \multirow{2}{*}{12} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  13:04:30.31  &  +30:58:55.08  &  20.30 $\pm$ 0.04  &  2.69 $\pm$ 5.42  &  -25.1 $\pm$ 5.42  & & &\\
 
\multirow{2}{*}{J1306+5925}  &  13:06:04.55  &  +59:25:09.47  &  19.75 $\pm$ 0.01  &  -0.94 $\pm$ 3.73  &  -58.89 $\pm$ 3.73  &  \multirow{2}{*}{63.1} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  13:06:06.71  &  +59:26:10.31  &  17.51 $\pm$ 0.01  &  3.34 $\pm$ 2.81  &  -62.99 $\pm$ 2.81  & & &\\
 
\multirow{2}{*}{J1309+5503}  &  13:09:54.23  &  +55:03:39.23  &  18.64 $\pm$ 0.01  &  52.11 $\pm$ 3.18  &  -27.57 $\pm$ 3.18  &  \multirow{2}{*}{13} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  13:09:55.67  &  +55:03:38.51  &  17.96 $\pm$ 0.01  &  51.32 $\pm$ 2.89  &  -29.21 $\pm$ 2.89  & & &\\
 
\multirow{2}{*}{CDDS28 } & 13:10:12.28 & +44:47:28.3  &  17.84 $\pm$ 0.02  &  &  & \multirow{2}{*}{15.71} &  & \multirow{2}{*}{3} \\ 
 & 13:10:13.38 & +44:47:17.8  &  17.59 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{LP 096-66/65}  &  13:10:20.68  &  +61:17:49.4  &  20.86 $\pm$ 0.03  &    &    &  \multirow{2}{*}{18} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  13:10:22.01  &  +61:18:04.67  &  19.62 $\pm$ 0.02  &  -295.89 $\pm$ 3.78  &  37.62 $\pm$ 3.78  & & &\\
 
\multirow{2}{*}{J1311+1543}  &  13:11:21.60  &  +15:43:04.79  &  19.97 $\pm$ 0.02  &  -39.75 $\pm$ 4.99  &  -12.45 $\pm$ 4.99  &  \multirow{2}{*}{10} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  13:11:21.84  &  +15:42:56.52  &  19.89 $\pm$ 0.02  &  -39.74 $\pm$ 3.5  &  -10.71 $\pm$ 3.5  & & &\\
 
\multirow{2}{*}{J1313+2030}  &  13:13:32.13  &  +20:30:39.63  &  17.79 $\pm$ 0.01  &    &    &  \multirow{2}{*}{5.9} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  13:13:32.56  &  +20:30:39.42  &  17.47 $\pm$ 0.01  &  -32.15 $\pm$ 4.64  &  24.69 $\pm$ 4.64  & & &\\
 
\multirow{2}{*}{CDDS30 } & 13:14:21.70 & +30:50:51.4  &  18.20 $\pm$ 0.08  &  &  & \multirow{2}{*}{2.76} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 13:14:21.50 & +30:50:50.5  &  17.86 $\pm$ 0.04  &  & & & & \\ 
 
\multirow{2}{*}{J1314+1732}  &  13:14:26.40  &  +17:32:27.96  &  18.65 $\pm$ 0.01  &  -40.58 $\pm$ 2.79  &  -60.69 $\pm$ 2.79  &  \multirow{2}{*}{20} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  13:14:26.88  &  +17:32:09.24  &  16.24 $\pm$ 0.01  &  -39.92 $\pm$ 2.33  &  -59.62 $\pm$ 2.33  & & &\\
 
\multirow{2}{*}{CDDS31 } & 13:28:14.28 & +16:31:51.5  &  16.27 $\pm$ 0.02  &  &  & \multirow{2}{*}{1.32} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 13:28:14.36 & +16:31:50.9  &  17.65 $\pm$ 0.23  &  & & & & \\ 
 
\multirow{2}{*}{J1342+5938}  &  13:42:45.86  &  +59:38:31.37  &  19.53 $\pm$ 0.01  &    &    &  \multirow{2}{*}{2.2} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  13:42:46.12  &  +59:38:30.69  &  19.80 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{J1347+2512}  &  13:47:37.68  &  +25:12:33.11  &  19.36 $\pm$ 0.01  &  -61.68 $\pm$ 3.24  &  -20.32 $\pm$ 3.24  &  \multirow{2}{*}{21.4} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  13:47:39.12  &  +25:12:28.79  &  20.22 $\pm$ 0.02  &  -63.02 $\pm$ 3.54  &  -17.65 $\pm$ 3.54  & & &\\
 
\multirow{2}{*}{CDDS32 } & 13:57:13.14 & -06:59:13.7  &  19.25 $\pm$ 0.02  &  &  & \multirow{2}{*}{26.29} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 13:57:14.50 & -06:58:56.9  &  18.16 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{J1412+4216}  &  14:12:07.68  &  +42:16:27.12  &  15.82 $\pm$ 0.01  &  -81.41 $\pm$ 2.66  &  -62 $\pm$ 2.66  &  \multirow{2}{*}{13.6} & \multirow{2}{*}{Y} & \multirow{2}{*}{2}\\
 &  14:12:08.87  &  +42:16:24.59  &  18.45 $\pm$ 0.01  &  -80 $\pm$ 3.11  &  -58.14 $\pm$ 3.11  & & &\\
 
\multirow{2}{*}{J1424-0317}  &  14:24:22.32  &  -03:17:43.33  &  19.15 $\pm$ 0.01  &  -126.39 $\pm$ 3.53  &  10.98 $\pm$ 3.53  &  \multirow{2}{*}{86.4} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  14:24:28.07  &  -03:17:47.54  &  19.38 $\pm$ 0.01  &  -121.09 $\pm$ 3.86  &  2.74 $\pm$ 3.86  & & &\\
 
\multirow{2}{*}{J1432+0136}  &  14:32:59.99  &  +01:36:36.03  &  20.75 $\pm$ 0.03  &  -57.68 $\pm$ 5.83  &  -14.02 $\pm$ 5.83  &  \multirow{2}{*}{88.3} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  14:33:05.75  &  +01:36:26.82  &  21.23 $\pm$ 0.05  &  -59.53 $\pm$ 5.97  &  -11.54 $\pm$ 5.97  & & &\\
 
\multirow{2}{*}{L 151-81A/B}  &  14:58:06  &  -63:17.1  &      &    &    &  \multirow{2}{*}{2} & \multirow{2}{*}{N} &\multirow{2}{*}{4} \\
 &  14:58:06  &  -63:17.1  &      &    &    && & \\
 
\multirow{2}{*}{J1507+5210}  &  15:07:46.48  &  +52:10:02.13  &  16.92 $\pm$ 0.01  &    &   &  \multirow{2}{*}{5} & \multirow{2}{*}{N} & \multirow{2}{*}{3,4}\\
 &  15:07:46.79  &  +52:09:58.06  &  17.77 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J1515+1436}  &  15:15:07.92  &  +14:36:35.45  &  19.61 $\pm$ 0.01  &    &    &  \multirow{2}{*}{7.9} & \multirow{2}{*}{N} &\multirow{2}{*}{1,3} \\
 &  15:15:08.30  &  +14:36:40.89  &  17.97 $\pm$ 0.01  &  2.94 $\pm$ 2.69  &  -21.59 $\pm$ 2.69  & &  &\\
 
\multirow{2}{*}{J1544+2344}  &  15:44:03.12  &  +23:44:58.92  &  18.42 $\pm$ 0.01  &  109.51 $\pm$ 2.98  &  -25.95 $\pm$ 2.98  &  \multirow{2}{*}{17.7} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  15:44:03.35  &  +23:45:16.55  &  19.64 $\pm$ 0.01  &  104.42 $\pm$ 3.51  &  -32.08 $\pm$ 3.51  & & \multirow{2}{*}{N} &\\
 
\multirow{2}{*}{J1546+6159}  &  15:46:41.49  &  +61:59:01.57  &  18.62 $\pm$ 0.01  &    &    &  \multirow{2}{*}{7.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  15:46:41.80  &  +61:58:54.19  &  16.86 $\pm$ 0.01  &  15.49 $\pm$ 2.43  &  -27.45 $\pm$ 2.43  & &  &\\
 
\multirow{2}{*}{J1552+4731}  &  15:52:44.40  &  +47:31:24.06  &  18.96 $\pm$ 0.01  &    &    &  \multirow{2}{*}{9.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  15:52:45.19  &  +47:31:29.53  &  18.71 $\pm$ 0.01  &  -8.85 $\pm$ 3.47  &  -11.95 $\pm$ 3.47  & & &\\
 
\multirow{2}{*}{CDDS37 } & 16:26:50.11 & +48:28:27.9  &  19.62 $\pm$ 0.02  &  &  & \multirow{2}{*}{20.22} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 16:26:52.12 & +48:28:24.7  &  18.98 $\pm$ 0.01  &  & & & & \\ 
 
\multirow{2}{*}{CDDS38 } & 16:36:47.81 & +09:27:15.7  &  17.72 $\pm$ 0.01  &  &  & \multirow{2}{*}{10.12} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 16:36:47.33 & +09:27:08.4  &  19.54 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{CDDS39 } & 16:57:37.90 & +62:01:02.1  &  18.65 $\pm$ 0.01  &  &  & \multirow{2}{*}{25.47} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 16:57:34.39 & +62:00:55.9  &  18.53 $\pm$ 0.01  &  & & & & \\ 
 
\multirow{2}{*}{J1703+3304}  &  17:03:55.92  &  +33:04:38.28  &  18.81 $\pm$ 0.01  &  0.14 $\pm$ 3.4  &  -52.27 $\pm$ 3.4  &  \multirow{2}{*}{11.2} & \multirow{2}{*}{N} & \multirow{2}{*}{2,3}\\
 &  17:03:56.87  &  +33:04:35.75  &  18.13 $\pm$ 0.01  &  2.46 $\pm$ 3.14  &  -51.45 $\pm$ 3.14  & & &\\
 
\multirow{2}{*}{Gr 576/577}  &  17:05:30.45  &  +48:03:12.02  &  14.43 $\pm$ 0.01  &    &    &  \multirow{2}{*}{5.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{4}\\
 &  17:05:30.98  &  +48:03:09.93  &  14.40 $\pm$ 0.01  &    &    && & \\
 
\multirow{2}{*}{LP 567-39/38}  &  17:28:30.65  &  +07:21:12.57  &  19.02 $\pm$ 0.12  &    &    &  \multirow{2}{*}{2} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  17:28:30.78  &  +07:21:13.42  &  18.38 $\pm$ 0.02  &  -62.21 $\pm$ 2.47  &  -286.81 $\pm$ 2.47  && & \\
 
\multirow{2}{*}{CDDS41 } & 17:32:49.57 & +56:39:00.0  &  18.95 $\pm$ 0.02  &  &  & \multirow{2}{*}{2.36} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 17:32:49.32 & +56:38:58.8  &  19.12 $\pm$ 0.05  &  & & & & \\ 
 
\multirow{2}{*}{CDDS42 } & 17:55:59.57 & +48:43:59.9  &  19.21 $\pm$ 0.02  &  &  & \multirow{2}{*}{16.41} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 17:55:58.35 & +48:43:48.8  &  17.68 $\pm$ 0.01  &  & & & & \\ 
 
\multirow{2}{*}{G 206-17/18}  &  18:13:31.24  &  +32:48:31.7  &    &    &    &  \multirow{2}{*}{55} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  18:13:35.46  &  +32:48:43.7  &    &    &    & & &\\
 
\multirow{2}{*}{G 021-15}  &  18:27:13.08  &  +04:03:46.7  &    &    &    &  \multirow{2}{*}{58.6} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &    &    &    &    &    & & &\\
 
\multirow{2}{*}{J1848+6415}  &  18:48:09.57  &  +64:15:20.08  &  19.78 $\pm$ 0.01  &    &    &  \multirow{2}{*}{2.2} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  18:48:09.69  &  +64:15:17.96  &  19.26 $\pm$ 0.01  &  16.94 $\pm$ 4.95  &  -18.28 $\pm$ 4.95  & & \multirow{2}{*}{N} &\\
 
\multirow{2}{*}{CDDS43 } & 20:43:18.96 & +00:58:41.8  &  18.24 $\pm$ 0.02  &  &  & \multirow{2}{*}{19.13} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 20:43:17.93 & +00:58:30.5  &  18.59$\pm$0.02  &  & & & & \\ 
 
\multirow{2}{*}{J2044+4030}  &  20:44:00.72  &  +40:30:06.01  &  17.86 $\pm$ 0.01  &    &    &  \multirow{2}{*}{9.1} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  20:44:01.03  &  +40:30:14.39  &  15.32 $\pm$ 0.01  &  18.78 $\pm$ 2.54  &  46.88 $\pm$ 2.54  & & &\\
 
\multirow{2}{*}{J2047+0021}  &  20:47:11.28  &  +00:21:27.35  &  17.06 $\pm$ 0.01  &  -6.24 $\pm$ 2.51  &  -100.91 $\pm$ 2.51  &  \multirow{2}{*}{49.8} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  20:47:13.68  &  +00:22:03.6  &  18.21 $\pm$ 0.01  &  -8.64 $\pm$ 2.8  &  -95.31 $\pm$ 2.8  & & &\\
 
\multirow{2}{*}{J2054+0640}  &  20:54:33.50  &  +06:40:30.97  &  20.13 $\pm$ 0.02  &    &    &  \multirow{2}{*}{5} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  20:54:33.62  &  +06:40:26.23  &  20.10 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{GD 392}  &  21:00:21.51  &  +34:26:21.0  &    &    &    &  \multirow{2}{*}{45.8} & \multirow{2}{*}{N} &\multirow{2}{*}{4} \\
 &  21:00:25.17  &  +34:26:10.81  &    &    &    & & &\\
 
\multirow{2}{*}{J2102+1029}  &  21:02:57.74  &  +10:29:53.77  &  19.71 $\pm$ 0.01  &    &    &  \multirow{2}{*}{3.3} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  21:02:57.83  &  +10:29:50.85  &  20.12 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{J2106+0211}  &  21:06:43.92  &  +02:11:54.58  &  20.39 $\pm$ 0.02  &    &    &  \multirow{2}{*}{4.1} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  21:06:44.11  &  +02:11:57.26  &  19.85 $\pm$ 0.01  &  13.49 $\pm$ 2.99  &  7.8 $\pm$ 2.99  & & &\\
 
\multirow{2}{*}{J2109+1809}  &  21:09:25.46  &  +18:09:27.86  &  19.45 $\pm$ 0.01  &    &    &  \multirow{2}{*}{2.3} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  21:09:25.51  &  +18:09:30.13  &  20.59 $\pm$ 0.02  &    &    & & &\\
 
\multirow{2}{*}{J2115-0741}  &  21:15:07.43  &  -07:41:51.54  &  17.44 $\pm$ 0.01  &  -25.33 $\pm$ 2.86  &  -117 $\pm$ 2.86  &  \multirow{2}{*}{17} &\multirow{2}{*}{N}  & \multirow{2}{*}{2}\\
 &  21:15:07.43  &  -07:41:34.51  &  16.78 $\pm$ 0.01  &  -30.12 $\pm$ 2.78  &  -117.74 $\pm$ 2.78  & & &\\
 
\multirow{2}{*}{CDDS44 } & 21:16:07.27 & +00:45:03.1  &  18.67 $\pm$ 0.01  &  &  & \multirow{2}{*}{2.06} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 21:16:07.20 & +00:45:01.3  &  18.96 $\pm$ 0.07  &  & & & & \\ 
 
\multirow{2}{*}{J2124-1620}  &  21:24:32.52  &  -16:20:21.94  &  16.12 $\pm$ 0.01  &    &    &  \multirow{2}{*}{8.3} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  21:24:32.59  &  -16:20:13.66  &  17.71 $\pm$ 0.01  &  -28.44 $\pm$ 2.45  &  -13.8 $\pm$ 2.45  & & &\\
 
\multirow{2}{*}{G 261-43}  &  21:26:57.69  &  +73:38:43.6  &  13.96 $\pm$ 0.01  &  53.42 $\pm$ 2.55  &  -288.79 $\pm$ 2.55  &  \multirow{2}{*}{1.4} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &    &    &      &     &    & & &\\
 
\multirow{2}{*}{CDDS45 } & 21:36:48.79 & +06:43:20.2  &  17.94 $\pm$ 0.02  &  &  & \multirow{2}{*}{3.44} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 21:36:48.98 & +06:43:18.2  &  19.35 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{CDDS46 } & 21:44:56.12 & +48:23:52.9  &  18.74 $\pm$ 0.01  &  &  & \multirow{2}{*}{14.67} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 21:44:57.39 & +48:23:45.5  &  19.49 $\pm$ 0.02  &  & & & & \\ 
 
\multirow{2}{*}{CDDS47 } & 21:53:09.89 & +46:19:02.7  &  17.72 $\pm$ 0.01  &  &  & \multirow{2}{*}{25.68} & \multirow{2}{*}{N}  & \multirow{2}{*}{3} \\ 
 & 21:53:08.90 & +46:18:39.1  &  19.08 $\pm$ 0.01  &  & & & & \\ 
 
\multirow{2}{*}{J2155+0315}  &  21:55:34.75  &  +03:15:39  &  19.32 $\pm$ 0.01  &    &    &  \multirow{2}{*}{3.1} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  21:55:34.94  &  +03:15:40.32  &  19.15 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J2222-0828}  &  22:22:36.31  &  -08:28:07.96  &  16.38 $\pm$ 0.01  &    &    &  \multirow{2}{*}{4.3} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  22:22:36.55  &  -08:28:06  &  17.07 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J2223+2201}  &  22:23:01.60  &  +22:01:31.36  &  15.59 $\pm$ 0.01  &    &    &  \multirow{2}{*}{6.6} & \multirow{2}{*}{N} & \multirow{2}{*}{1,3}\\
 &  22:23:01.72  &  +22:01:24.95  &  16.00 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J2224+2315}  &  22:24:26.92  &  +23:15:36.03  &  17.83 $\pm$ 0.01  &    &    &  \multirow{2}{*}{2.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  22:24:27.09  &  +23:15:37.47  &  17.16 $\pm$ 0.01  &    &    && & \\
 
\multirow{2}{*}{J2227-0713}  &  22:27:27.81  &  -07:13:03.3  &  18.87 $\pm$ 0.01  &    &    &  \multirow{2}{*}{4.5} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  22:27:28.05  &  -07:13:05.97  &  19.19 $\pm$ 0.01  &  13.74 $\pm$ 2.71  &  -14.34 $\pm$ 2.71  & & &\\
 
\multirow{2}{*}{SSSPM J2231-7514}  &  22:30:96.61  &  -75:13:49.36  &    &    &    &  \multirow{2}{*}{93} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  22:30:33.14  &  -75:15:18.43  &    &    &    & & &\\
 
\multirow{2}{*}{J2236+2928}  &  22:36:02.87  &  +29:28:51.34  &  18.48 $\pm$ 0.01  &    &    &  \multirow{2}{*}{9.9} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  22:36:03.48  &  +29:28:45.08  &  20.08 $\pm$ 0.02  &  7.74 $\pm$ 3.25  &  0.99 $\pm$ 3.25  & & &\\
 
\multirow{2}{*}{HS 2240+1234}  &  22:42:30.23  &  +12:50:02.39  &  16.47 $\pm$ 0.01  &  -33.86 $\pm$ 2.76  &  -72.6 $\pm$ 2.76  &  \multirow{2}{*}{12.1} & \multirow{2}{*}{N} & \multirow{2}{*}{3,4}\\
 &  22:42:31.19  &  +12:50:04.91  &  16.19 $\pm$ 0.01  &  -32.17 $\pm$ 2.73  &  -75.96 $\pm$ 2.73  && & \\
 
\multirow{2}{*}{J2259+1404}  &  22:59:32.20  &  +14:04:39.28  &  16.35 $\pm$ 0.01  &    &    &  \multirow{2}{*}{9.1} & \multirow{2}{*}{Y} & \multirow{2}{*}{1,3}\\
 &  22:59:32.73  &  +14:04:44.25  &  18.58 $\pm$ 0.01  &  26.63 $\pm$ 3.25  &  -13.33 $\pm$ 3.25  & & &\\
 
\multirow{2}{*}{J2302+2430}  &  23:02:49.43  &  +24:30:28.07  &  18.16 $\pm$ 0.01  &  -48.66 $\pm$ 2.81  &  -127.1 $\pm$ 2.81  &  \multirow{2}{*}{19.9} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  23:02:50.40  &  +24:30:13.67  &  18.49 $\pm$ 0.01  &  -51.55 $\pm$ 3  &  -126.52 $\pm$ 3  & & &\\
 
\multirow{2}{*}{J2303-0755}  &  23:03:27.83  &  -07:55:04.72  &  18.14 $\pm$ 0.01  &  43.59 $\pm$ 2.54  &  6.37 $\pm$ 2.54  &  \multirow{2}{*}{7.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  23:03:28.08  &  -07:54:57.88  &  18.16 $\pm$ 0.01  &  42.87 $\pm$ 2.57  &  9.42 $\pm$ 2.57  && & \\
 
\multirow{2}{*}{LP 701-69/70}  &  23:04:19.09  &  -07:01:26.71  &  17.19 $\pm$ 0.02  &  238.95 $\pm$ 2.3  &  -224.63 $\pm$ 2.3  &  \multirow{2}{*}{26} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  23:04:19.65  &  -07:01:52.03  &  19.98 $\pm$ 0.03  &    &    & & &\\
 
\multirow{2}{*}{J2317+5550}  &  23:17:57.26  &  +55:50:34.58  &  18.72 $\pm$ 0.01  &    &    &  \multirow{2}{*}{8.7} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  23:17:57.59  &  +55:50:26.26  &  15.27 $\pm$ 0.01  &  11.48 $\pm$ 2.49  &  10.83 $\pm$ 2.49  && & \\
 
\multirow{2}{*}{J2319+3426}  &  23:19:41.35  &  +34:26:14.24  &  17.24 $\pm$ 0.01  &    &    &  \multirow{2}{*}{5.1} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  23:19:41.44  &  +34:26:09.31  &  17.57 $\pm$ 0.01  &  -40.89 $\pm$ 5.85  &  -78.44 $\pm$ 5.85  & & &\\
 
\multirow{2}{*}{GD 559}  &  23:21:17.28  &  +69:26:22.52  &  15.14 $\pm$ 0.04  &  -132.02 $\pm$ 2.73  &  -8.32 $\pm$ 2.73  &  \multirow{2}{*}{28.7} & \multirow{2}{*}{Y} & \multirow{2}{*}{4}\\
 &  23:21:17.24  &  +69:25:53.8  &  18.23 $\pm$ 0.04  &  -133.94 $\pm$ 3.07  &  -5.89 $\pm$ 3.07  && & \\
 
\multirow{2}{*}{J2326-0023}  &  23:26:58.79  &  -00:23:39.98  &  19.36 $\pm$ 0.01  &  53.95 $\pm$ 3.22  &  -30.73 $\pm$ 3.22  &  \multirow{2}{*}{9.5} & \multirow{2}{*}{N} & \multirow{2}{*}{2}\\
 &  23:26:59.27  &  -00:23:48.1  &  17.51 $\pm$ 0.01  &  55.15 $\pm$ 2.67  &  -28.99 $\pm$ 2.67  & & &\\
 
\multirow{2}{*}{J2332+4917}  &  23:32:46.24  &  +49:17:09.13  &  18.76 $\pm$ 0.01  &    &    &  \multirow{2}{*}{3} & \multirow{2}{*}{N} & \multirow{2}{*}{1,3}\\
 &  23:32:46.27  &  +49:17:12.08  &  18.67 $\pm$ 0.01  &    &    & & &\\
 
\multirow{2}{*}{J2337+2123}  &  23:37:06.24  &  +21:23:23.28  &  18.66 $\pm$ 0.01  &  70.57 $\pm$ 2.79  &  33.98 $\pm$ 2.79  &  \multirow{2}{*}{14.2} & \multirow{2}{*}{N} & \multirow{2}{*}{1}\\
 &  23:37:07.19  &  +21:23:20.75  &  19.67 $\pm$ 0.01  &  75.8 $\pm$ 3.19  &  31.53 $\pm$ 3.19  & & &\\
 
\multirow{2}{*}{J2345+3507}  &  23:45:26.40  &  +35:07:53.75  &  20.22 $\pm$ 0.03  &  -36.88 $\pm$ 4.09  &  -36.03 $\pm$ 4.09  &  \multirow{2}{*}{9.3} & \multirow{2}{*}{N} &  \multirow{2}{*}{1}\\
 &  23:45:26.88  &  +35:07:46.91  &  17.57 $\pm$ 0.01  &  -38.49 $\pm$ 2.38  &  -36.27 $\pm$ 2.38  & & &\\
 
\multirow{2}{*}{LP 077-57/56}  &  23:54:07.98  &  +65:22:34.01  &    &    &    &  \multirow{2}{*}{3} & \multirow{2}{*}{N} & \multirow{2}{*}{4}\\
 &  23:54:07.71  &  +65:22:31.48  &    &    &    & & &\\
 
\multirow{2}{*}{J2355+1708}  &  23:55:15.36  &  +17:08:06.72  &  18.23 $\pm$ 0.01  &  51.75 $\pm$ 2.69  &  2.94 $\pm$ 2.69  &  \multirow{2}{*}{24.4} & \multirow{2}{*}{Y} & \multirow{2}{*}{1}\\
 &  23:55:15.36  &  +17:08:30.83  &  16.22 $\pm$ 0.01  &  53.01 $\pm$ 2.33  &  4.36 $\pm$ 2.33  & & &\\
\enddata 
\tablerefs{1--This work, 2--Paper I, 3--\citet{baxter14}, 4--Literature, see Paper I for references}
\tablecomments{The full table may be found in the online edition of the journal. The WDs in each pair are ordered by RA, regardless of the ``A'' or ``B'' designation that may exist in the literature.}
\end{deluxetable*} 

